Nominal Metaphor Generation with Multitask Learning

Metaphor generation is a challenging task which can impact many downstream tasks such as improving user satisfaction with dialogue systems and story generation. This paper tackles the problem of Chinese nominal metaphor generation by introducing a multitask metaphor generation framework with self-training and metaphor identification mechanisms. Self-training addresses the data scarcity issue of metaphor datasets. That is, instead of solely relying on labelled metaphor datasets which are usually small in size, self-training helps identify potential metaphors from a large-scale unlabelled corpus for metaphor generation. The metaphor weighting mechanism enables our model to focus on the metaphor-related parts of the input (e.g., the comparison of the metaphor and comparator) during model learning and thus improves the metaphoricity of the generated metaphors. Our model is trained on an annotated corpus consisting of 6.3k sentences that contain diverse metaphorical expressions. Experimental results show that our model is able to generate metaphors with better readability and creativity compared to the baseline models, even in the situation where training data is insufficient.

==> experiment.tex <==
\section{Experiment}

\subsection{dataset}
To train our multitask framework, we construct two datasets: a supervised Chinese NM Corpora (CMC) and a large-scale unsupervised Chinese Literature Corpora (CLC).

\noindent \textbf{\CMC} The annotation of the CMC consists of three steps: 1) we collecting 55,000 Chinese sentences from essays, articles and novels; 2) we employ three annotators to label each sentence as a NM or not; 3) we take the majority agreement as the final label for each sentence. 



\subsection{Baselines}
Chinese NMs generation is a novel task, we select three general generative models and a English Simile generation method as baselines.

\textbf{SeqGAN: } Sequence Generative adversarial network with a generator implemented by LSTM metwork and a discriminator implemented by CNN network. The generator of SeqGAN is 


